A Generative Framework for Personalized Learning and Estimation: Theory, Algorithms, and Privacy

A distinguishing characteristic of federated learning is that the (local) client data could have statistical heterogeneity. This heterogeneity has motivated the design of personalized learning, where individual (personalized) models are trained, through collaboration. There have been various personalization methods proposed in literature, with seemingly very different forms and methods ranging from use of a single global model for local regularization and model interpolation, to use of multiple global models for personalized clustering, etc. In this work, we begin with a generative framework that could potentially unify several different algorithms as well as suggest new algorithms. We apply our generative framework to personalized estimation, and connect it to the classical empirical Bayes' methodology. We develop private personalized estimation under this framework. We then use our generative framework for learning, which unifies several known personalized FL algorithms and also suggests new ones; we propose and study a new algorithm AdaPeD based on a Knowledge Distillation, which numerically outperforms several known algorithms. We also develop privacy for personalized learning methods with guarantees for user-level privacy and composition. We numerically evaluate the performance as well as the privacy for both the estimation and learning problems, demonstrating the advantages of our proposed methods.

==> app_est_mixture.tex <==
%\cred{this is about discrete prior model...}

\cred{\hrule}

Consider a set of $m$ clients, where the $i$-th client has a local dataset $X_{i}=\left(X_{i1},\ldots,X_{in}\right)$ of $n$ samples for $i\in[m]$, where $X_{ij}\in\mathbb{R}^{d}$. The local samples $X_i$ of the $i$-th client are drawn i.i.d. from a Gaussian distribution with unknown mean $\theta_i$ and known variance $\sigma_x^2\mathbb{I}_{d\times d}$.


In this section, we assume that the personalized models $\theta_1,\ldots,\theta_m$ are drawn i.i.d. from a discrete distribution $P=\left[p_1,\ldots,p_k\right]$ for given $k$ candidates $\mu_1,\ldots,\mu_k\in\mathbb{R}^{d}$. In other works, $\Pr[\theta_i=\mu_l]=p_l$ for $l\in[k]$ and $i\in[m]$. The goal of each client is to estimate her personalized model $\lbrace\theta_i\rbrace$ by $\htheta_i$ that minimizes the mean square error defined as follows:
\begin{equation}
MSE = \mathbb{E}_{\lbrace\theta_i,X_i\rbrace}\left[\|\theta_i-\hat{\theta}_i\|^2\right],    
\end{equation}
where the expectation is taken with respect to the personalized models $\theta_i\sim P$ and the local samples $\lbrace X_{ij}\sim\mathcal{N}(\theta_i,\sigma_x^2\mathbb{I}_{d\times d}) \rbrace$. Furthermore, $\hat{\theta}_i$ denotes the estimate of the personalized model $\theta_i$ for $i\in[m]$. 


First, we start with a simple case when the clients have perfect knowledge of the prior distribution, i.e., the $i$-th client knows the $k$ possible vectors $\mu_1,\ldots,\mu_k$ and the prior distribution $P=\left[p_1,\ldots,p_k\right]$. In this case, the $i$-th client does not need the data of the other clients as she has a perfect knowledge about the prior distribution. 

\begin{theorem}\label{thm:discrete_perfect}
For given a perfect knowledge $P=[p_1,\ldots,p_k]$ and $\mu_1,\ldots,\mu_k$, the optimal personalized estimator that minimizes the MSE is given by:
\begin{equation}\label{eqn:discrete_perfect_estimator}
\hat{\theta}_i =\sum_{l=1}^{k}\alpha_{l}^{(i)}\mu_l,
\end{equation}
where $\alpha_{l}^{(i)}=\frac{p_l\exp{\left(-\frac{\sum_{j=1}^{n}\|X_{ij}-\mu_l\|^2}{2\sigma_x^2}\right)}}{\sum_{s=1}^{k}p_s\exp{\left(-\frac{\sum_{j=1}^{n}\|X_{ij}-\mu_s\|^2}{2\sigma_x^2}\right)}}$ denotes the weight associated to the prior model $\mu_l$ for $l\in[k]$.
\end{theorem}
\begin{proof}
Let $\theta_i\sim P$, where $P=[p_1,\ldots,p_k]$ and $p_l=\Pr[\theta_i=\mu_l]$ for $l\in[k]$. The goal is to design an estimator $\hat{\theta}_i$ that minimizes the MSE given by:
\begin{equation}
    MSE = \mathbb{E}_{\theta_i\sim P}\mathbb{E}_{\lbrace X_{ij}\sim\mathcal{N}(\theta_i,\sigma_x^2)\rbrace}\left[\|\hat{\theta}_i-\theta_i\|^2\right].
\end{equation}
Let $X_i=(X_{i1},\ldots,X_{in})$. By following the standard proof of the minimum MSE, we get that:
\begin{equation}
\begin{aligned}
\mathbb{E}_{\theta_i}\mathbb{E}_{X_i}\left[\|\hat{\theta}_i-\theta_i\|^2\right]&= \mathbb{E}_{X_i}\mathbb{E}_{\theta_i|X_i}\left[\left.\|\hat{\theta}_i-\mathbb{E}[\theta_i|X_i]+\mathbb{E}[\theta_i|X_i]-\theta_i\|^2\right|X_i\right]\\
& = \mathbb{E}_{X_i}\mathbb{E}_{\theta_i|X_i}\left[\left.\|\mathbb{E}[\theta_i|X_i]-\theta_i\|^2\right|X_i\right]+ \mathbb{E}_{X_i}\mathbb{E}_{\theta_i|X_i}\left[\left.\|\mathbb{E}[\theta_i|X_i]-\hat{\theta}_i\|^2\right|X_i\right] \\
&\geq \mathbb{E}_{X_i}\mathbb{E}_{\theta_i|X_i}\left[\left.\|\mathbb{E}[\theta_i|X_i]-\theta_i\|^2\right|X_i\right],
\end{aligned}
\end{equation}
where the last inequality is achieved with equality when $\hat{\theta}_i=\mathbb{E}[\theta_i|X_i]$. The distribution on $\theta_i$ given the local dataset $X_i$ is given by:
\begin{equation}
\begin{aligned}
\Pr[\theta_i=\mu_l|X_i] &= \frac{f(X_i|\theta_i=\mu_l)\Pr[\theta_i=\mu_l]}{f(X_i)}\\  
&= \frac{f(X_i|\theta_i=\mu_l)\Pr[\theta_i=\mu_l]}{\sum_{s=1}^{k}f(X_i|\theta_i=\mu_s)\Pr[\theta_i=\mu_s]}\\
&= \frac{p_l \exp\left(-\frac{\sum_{j=1}^{n}\|X_{ij}-\mu_l\|^2}{2\sigma_x^2}\right)}{\sum_{s=1}^{k}p_s\exp\left(-\frac{\sum_{j=1}^{n}\|X_{ij}-\mu_s\|^2}{2\sigma_x^2}\right)} =\alpha_l^{(i)}
\end{aligned}
\end{equation}
As a result, the optimal estimator is given by:
\begin{equation}
\hat{\theta}_i= \mathbb{E}[\theta_i|X_i]=\sum_{l=1}^{k}\alpha_{l}^{(i)} \mu_l. 
\end{equation}
This completes the proof of Theorem~\ref{thm:discrete_perfect}.
\end{proof}










%
%Consider a set of $m$ clients, where the $i$-th client has a local dataset $x_{i}=\left(x_{i1},\ldots,x_{in}\right)$ of $n$ samples for $i\in[m]$, where $x_{ij}\in\mathbb{R}^{d}$. The local samples $x_i$ of the $i$-th client are drawn i.i.d. from a Gaussian distribution with unknown mean $\theta_i$ and known variance $\sigma_x^2\mathbb{I}_{d\times d}$.
%In this section, we assume that the personalized models $\theta_1,\ldots,\theta_m$ are drawn i.i.d. from a discrete distribution $P=\left[p_1,\ldots,p_k\right]$ for given $k$ candidates $\mu_1,\ldots,\mu_k\in\mathbb{R}^{d}$. In other works, $\Pr[\theta_i=\mu_l]=p_l$ for $l\in[k]$ and $i\in[m]$. The goal of each client is to estimate her personalized model $\lbrace\theta_i\rbrace$ that minimizes the mean square error defined as follows:
%\begin{equation}
%MSE = \mathbb{E}_{\lbrace\theta_i,x_i\rbrace}\left[\|\theta_i-\hat{\theta}_i\|^2\right],    
%\end{equation}
%where the expectation is taken with respect to the personalized models $\lbrace\theta_i\sim P\rbrace$ and the local samples $\lbrace x_{ij}\sim\mathcal{N}(\theta_i,\sigma_x^2\mathbb{I}_{d\times d}) \rbrace$, and $\hat{\theta}_i$ denotes the estimate of the personalized model $\theta_i$. 
%
%First, we start with a simple case when the clients have perfect knowledge of the prior distribution, i.e., the $i$-th client knows the $k$ possible vectors $\mu_1,\ldots,\mu_k$ and the prior distribution $P=\left[p_1,\ldots,p_k\right]$. In this case, the $i$-th client does not need the data of the other clients as she has a perfect knowledge about the prior distribution. 
%\begin{theorem}~\label{thm:discrete_perfect}
%For given a perfect knowledge $P=[p_1,\ldots,p_k]$ and $\mu_1,\ldots,\mu_k$, the optimal personalized estimator that minimizes the MSE is given by:
%\begin{equation}\label{eqn:discrete_perfect_estimator}
%\hat{\theta}_i =\sum_{l=1}^{k}\alpha_{l}^{(i)}\mu_l,
%\end{equation}
%where $\alpha_{l}^{(i)}=\frac{p_l\exp{\left(-\frac{\sum_{j=1}^{n}\|x_{ij}-\mu_l\|^2}{2\sigma_x^2}\right)}}{\sum_{s=1}^{k}p_s\exp{\left(-\frac{\sum_{j=1}^{n}\|x_{ij}-\mu_s\|^2}{2\sigma_x^2}\right)}}$ denotes the weight associated to the prior model $\mu_l$ for $l\in[k]$.
%\end{theorem}
%The proof of Theorem~\ref{thm:discrete_perfect} is presented in Appendix~\ref{app:cluster_perfect}. 


The optimal personalized estimation in~\eqref{eqn:discrete_perfect_estimator} is a weighted summation over all possible candidates vectors $\mu_1,\ldots,\mu_k$, where the weight $\alpha_{l}^{(i)}$ increases if the prior $p_l$ increases and/or the local samples $\lbrace X_{ij}\rbrace$ are close to the model $\mu_l$ for $l\in[k]$. Observe that the optimal estimator $\hat{\theta}_i$ in Theorem~\ref{thm:discrete_perfect} that minimizes the MSE is completely different from the local estimator $\left(\frac{1}{n}\sum_{j=1}^{n}X_{ij}\right)$. Furthermore, it is easy to see that the local estimator has a MSE given by $\left(\frac{d\sigma_x^2}{n}\right)$ that increases linearly with the data dimension $d$. On the other hand, the MSE of the optimal estimator in Theorem~\ref{thm:discrete_perfect} is a function of the prior distribution $P=[p_1,\ldots,p_k]$, the prior vectors $\mu_1,\ldots,\mu_k$, and the local variance $\sigma_x^2$. 

%We evaluate numerically the gap between the MSE of the local estimator $\left(\frac{1}{n}\sum_{j=1}^{n}x_{ij}\right)$ and the personalized estimator in~\eqref{eqn:discrete_perfect_estimator} in Section~\ref{sec:experiments}. \cred{do we give this result?} 

Now, we consider the more practical case when the prior distribution $P=[p_1,\ldots,p_k]$ and the candidates $\mu_1,\ldots,\mu_k$ are unknown to the clients. In this case, the clients collaborate with each other by their local data to estimate the priors $P$ and $\mu_1,\ldots,\mu_k$, and then, each client uses the estimated priors to design her personalized model as in~\eqref{eqn:discrete_perfect_estimator}. 

We present Algorithm~\ref{algo:cluster} based on alternating minimization. The algorithm starts from initializing the local models $\lbrace\theta_{i}^{(0)}=\frac{1}{n}\sum_{j=1}^{n}X_{ij}\rbrace$. Then, the algorithm works in rounds alternating between estimating the priors $P^{(t+1)}=[p_1^{(t+1)},\ldots,p_k^{(t+1)}]$, $\mu_1^{(t+1)},\ldots,\mu_k^{(t+1)}$ for given local models $\lbrace \theta_i^{(t)}\rbrace$ and estimating the personalized models $\lbrace \theta_i^{(t+1)}\rbrace$ for given the global priors $P^{(t+1)}$ and $\mu_1^{(t+1)},\ldots,\mu_1^{(t+1)}$. Observe that for given the prior information $P^{(t)},\lbrace \mu_l^{t}\rbrace$, each client updates her personalized model in Step~\ref{step:personal_update} which is the optimal estimator for given priors according to Theorem~\ref{thm:discrete_perfect}. On the other hand, for given the personalized models $\lbrace \theta_i^{(t)}\rbrace$, we estimate the priors $P^{(t)},\lbrace \mu_l^{t}\rbrace$ using clustering algorithm with $k$ sets in Step~\ref{step:clustering}. The algorithm $\mathsf{Cluster}$ has input of $m$ vectors $a_1,\ldots,a_m$ and an integer $k$. The goal of the algorithm $\mathsf{Cluster}$ is to generate a set of $k$ cluster centers $\mu_1,\ldots,\mu_k$ that minimizes $\sum_{i=1}^{m}\min_{l\in k}\|a_i-\mu_l\|^2$. Furthermore, these clustering algorithms can also return the prior distribution $P$, by setting $p_l=\frac{|\mathcal{S}_l|}{m}$, where $\mathcal{S}_l\subset \lbrace a_1,\ldots,a_m\rbrace$ denotes the set of vectors that are belongs to the $l$-th cluster. There are lots of algorithms that do clustering, but perhaps, Lloyd’s algorithm~\cite{lloyd1982least} and Ahmadian~\cite{ahmadian2019better} are the most common algorithms for $k$-mean clustering. Our Algorithm~\ref{algo:cluster} can work with any clustering algorithm.

\begin{algorithm}[H]
			\caption{Alternating Minimization Estimation}
			{\bf Input:} Number of iterations $T$, local datasets $(X_{i1},\ldots,X_{in})$ for $i\in[m]$.\\
			\vspace{-0.3cm}
			\begin{algorithmic}[1] 	\label{algo:cluster}
			\STATE \textbf{Initialize} $\theta_i^{0}=\frac{1}{n}\sum_{j=1}^{n}X_{ij}$  for $i\in[m]$.
			\FOR{$t=1$ \textbf{to} $T$}
			\STATE~\label{step:clustering} \textbf{Update the priors:}
			$P^{(t)},\mu_1^{(t)},\ldots,\mu_k^{(t)}\gets \mathsf{Cluster}\left(\theta_1^{(t-1)},\ldots,\theta_m^{(t-1)},k\right)$
			\FOR {$i=1$ \textbf{to} $m$:}
			\STATE ~\label{step:personal_update} \textbf{Update the personalized model:} $\theta_i^{t}\gets \sum_{l=1}^{k}\alpha_{l}^{(i)}\mu_l^{(t)}$ and $\alpha_{l}^{(i)}\gets\frac{p_l^{(t)}\exp{\left(-\frac{\sum_{j=1}^{n}\|X_{ij}-\mu_l^{(t)}\|^2}{2\sigma_x^2}\right)}}{\sum_{s=1}^{k}p_s^{(t)}\exp{\left(-\frac{\sum_{j=1}^{n}\|X_{ij}-\mu_s^{(t)}\|^2}{2\sigma_x^2}\right)}}$
			\ENDFOR
			\ENDFOR
			\end{algorithmic}
			{\bf Output:} Personalized models $\theta_1^{T},\ldots,\theta_m^{T}$.
\end{algorithm}

\textbf{Private/Communication Estimation:} In the personalized Algorithm~\ref{algo:cluster}, each client shares her personalized estimator $\theta_{i}^{(t)}$ to the server at each iteration which is not communication-efficient and violates the privacy. In this section we present ideas on how to design communication-efficient and/or private Algorithms for personalized estimate with discrete priors.  

\begin{lemma}~\label{lemm:concentration}
Let $\mu_1,\ldots\mu_k\in\mathcal{B}(r)$ are unknown means. Let $\theta_1,\ldots,\theta_m\sim P=[p_1,\ldots,p_k]$, where $p_l=\Pr[\theta_i=\mu_l]$. For $i\in[m]$, let $X_{i1},\ldots,X_{in}\sim\mathcal{N}(\theta_i,\sigma_x^2)$. For all $i\in[m]$, we have that:
\begin{equation}
\|\frac{1}{n}\sum_{j=1}^{n}X_{ij}\|_2\leq 4\sqrt{d\frac{\sigma_x^2}{n}}+2\sqrt{\log(m^2n)\frac{\sigma_x^2}{n}}+r,    
\end{equation}
with probability at least $1-\frac{1}{mn}$.
\end{lemma}
\begin{proof}
Observe that the vector $(\overline{X}_i-\theta_i)=\frac{1}{n}\sum_{i=1}^{n}X_{ij}-\theta_i$ is a sub-Gaussian random vector with proxy $\frac{\sigma_x^2}{n}$. As a result, we have that:
\begin{equation}
\|\overline{X}_i-\theta_i\|_2\leq 4\sqrt{d\frac{\sigma_x^2}{n}}+2\sqrt{\log(1/\eta)\frac{\sigma_x^2}{n}},
\end{equation} 
with probability at least $1-\eta$ from~\cite{wainwright2019high}. Since $\mu_1,\ldots,\mu_k\in\mathcal{B}(r)$, we have that:
\begin{equation}
\|\overline{X}_i\|_2\leq 4\sqrt{d\frac{\sigma_x^2}{n}}+2\sqrt{\log(1/\eta)\frac{\sigma_x^2}{n}}+r,
\end{equation}
with probability $1-\eta$ from the triangular inequality. Thus, by choosing $\eta = \frac{1}{m^2n}$ and using the union bound, this completes the proof of Lemma~\ref{lemm:concentration}.
\end{proof}
Lemma~\ref{lemm:concentration} shows that the average of the local samples $\lbrace\overline{x}_i\rbrace$ has a bounded $\ell_2$ norm with high probability. Thus, we can design a communication-efficient estimation Algorithm as follows: Each client clips her personal model $\theta_i^{(t)}$ within radius $4\sqrt{d\frac{\sigma_x^2}{n}}+2\sqrt{\log(m^2n)\frac{\sigma_x^2}{n}}+r$. Then, each client applies a vector-quantization scheme (e.g.,~\cite{bernstein2018signsgd,alistarh2017qsgd,girgis2021shuffled}) to the clipped vector before sending it to the server. 

To design a private estimation algorithm with discrete priors, each client clips her personal model $\theta_{i}^{(t)}$ within radius $4\sqrt{d\frac{\sigma_x^2}{n}}+2\sqrt{\log(m^2n)\frac{\sigma_x^2}{n}}+r$. Then, we can use a differentially private algorithm for clustering (see e.g.,~\cite{stemmer2020locally} for clustering under LDP constraints and~\cite{ghazi2020differentially} for clustering under central DP constraints.).  Since, we run $T$ iterations in Algorithm~\ref{algo:cluster}, we can obtain the final privacy analysis $(\epsilon,\delta)$ using the strong composition theorem~\cite{dwork2014algorithmic}.


==> app_learn_logistic.tex <==
As described in Section~\ref{sec:learning}, by taking $\bbP(\Gamma)\equiv\calN(\vct{\mu},\sigmatheta^2\bbI_d)$ and $p_{\vct{\theta}_i}(Y_{ij}|X_{ij})=\sigma(\langle \vct{\theta}_i, X_{ij} \rangle)^{Y_{ij}}(1-\sigma(\langle \vct{\theta}_i, X_{ij} \rangle))^{(1-Y_{ij})}$, where $\sigma(z)=\nicefrac{1}{1+e^{-z}}$ for any $z\in\bbR$, then the overall optimization problem becomes:

%$f_i(\vct{\theta}_i)$ is the cross-entropy loss (or the logistic loss) as in the case of logistic regression.
%
%Now we write down the full objective function for linear regression by taking $\bbP(\Gamma)\equiv\calN(\vct{\mu},\sigmatheta^2\bbI_d)$ and $p_{\vct{\theta}_i}(Y_{ij}|X_{ij})$ according to $\calN(\vct{\theta}_i,\sigma_x^2)$; the case of logistic regression can be similarly handled. Here, if we assume that in addition to $\vct{\mu}$, the other parameters $\sigmatheta,\sigma_x$ are also unknown, then we can also optimize over them. In this case, the overall optimization problem becomes:
\begin{align}\label{eqn:logistic-regression}
&\argmin_{\{\vct{\theta}_i\},\vct{\mu}, \sigmatheta}\sum_{i=1}^{m}\sum_{j=1}^{n}\left[Y_{ij}\log\left(\frac{1}{1+e^{-\langle\vct{\theta}_i,X_{ij}\rangle}}\right) + (1-Y_{ij})\log\left(\frac{1}{1+e^{\langle\vct{\theta}_i,X_{ij}\rangle}}\right)\right] \notag \\
&\hspace{5cm} +\frac{md}{2}\log(2\pi\sigma_{\vct{\theta}}^2)+\sum_{i=1}^{m}\frac{\|\vct{\mu}-\vct{\theta}_i\|_2^2}{2\sigma_{\vct{\theta}}^2}.
\end{align}

%\textbf{General Logistic Regression Setting.} Considering a general cases/datasets, it is useful to derive the prior as a generating model for $\theta$. In particular, as in linear regression case, if we assume $\theta_i \sim N(\mu, \sigma_{\theta}^2\mathbb{I}_{dxd})$ we obtain the following MAP problem:  
%
%\begin{align*}
%	\hat{\theta}_1,\ldots,\hat{\theta}_m &= \argmax f_{\theta|\mathbf{X},\mathbf{Y}}\\
%	&= \argmin  \sum_{i=1}^m \sum_{j=1}^n \left( (y_j)\log\left(\frac{1}{1+e^{-\theta_i^Tx_j}}\right)+(1-y_j)\log\left(\frac{1}{1+e^{\theta_i^Tx_j}}\right) \right) \\
%	& \quad +\frac{md}{2}\log(2\pi\sigma_{\theta}^2)+\sum_{i=1}^{m}\frac{\|\mu-\theta_i\|^2}{2\sigma_{\theta}^2}.
%\end{align*}

When $\vct{\mu}$ and $\sigma_{\theta}^2$ are unknown, we would like to learn them by gradient descent, as in the linear regression case. The corresponding algorithm is described in Algorithm~\ref{algo:personalized_logsitic_regression}.

\begin{algorithm}
	\caption{Logistic Regression SGD}
	{\bf Input:} Number of iterations $T$, local datasets $(Y_i, X_i)$ for $i\in[m]$, learning rate $\eta$.\\
	\vspace{-0.3cm}
	\begin{algorithmic}[1] 	\label{algo:personalized_logsitic_regression}
		\STATE \textbf{Initialize} $\theta_i^{0}$  for $i\in[m]$, $\mu^0$, $\sigma_{\theta}^{2,0}$.
		\FOR{$t=1$ \textbf{to} $T$} 
		\STATE On Clients:
		\FOR {$i=1$ \textbf{to} $m$:}
		\STATE Receive and set $\mu_{i}^t = \mu^{t},\sigma^{2,t}_{\theta,i}=\sigma^{2,t}_{\theta}$
		\STATE \textbf{Update the personalized model:}\\ $\theta_i^{t}\gets\theta_{i}^{t-1}-\eta\left(\sum_{j=1}^{n}\nabla_{\theta_i^{t-1}}l_{CE}^{(p)}(\theta_i^{t-1}, (X_i^j,Y_i^j))+\frac{\mu_i^{t-1}-\theta_i^{t-1}}{\sigma_{\theta,i}^{2,t-1}}\right)$
		\STATE \textbf{Update local version of mean:} $\mu_i^{t}\gets\mu_i^{t-1}-\eta\left(\frac{\mu_i^{t-1}-\theta_i^{t-1}}{\sigma_{\theta,_i}^{2,t-1}}\right)$
		\STATE \textbf{Update global variance:} $\sigma^{2,t}_{\theta,_i}\gets\sigma^{2,t-1}_{\theta,_i}-\eta\left(\frac{d}{2\sigma_{\theta,i}^{2,t-1}}-\frac{\|\mu_i^{t-1}-\theta^{t-1}_i\|^2}{2(\sigma_{\theta,i}^{2,t-1})^2}\right)$
		\ENDFOR
		\STATE At the Server:
		\STATE \textbf{Aggregate mean:} $\mu^{t}=\frac{1}{m}\sum_{i=1}^{m}\mu_i^t$
		\STATE \textbf{Aggregate global variance:} $\sigma^{2,t}_{\theta}= \frac{1}{m}\sum_{i=1}^{m}\sigma^{2,t}_{\theta,i}$
		\STATE Broadcast $\mu^{t},\sigma^{2,t}_{\theta}$ 
		\ENDFOR
	\end{algorithmic}
	{\bf Output:} Personalized models $\theta_1^{T},\ldots,\theta_m^{T}$.
\end{algorithm}

%\textbf{A simplified version that connects to the Bernoulli model.} An interesting observation can be made when we examine a simplified version of logistic regression which is considered in \cite{duchi2019lower}. Consider a simplified logistic regression problem as in \cite{duchi2019lower}, where a client $i$ possesses local dataset tuple $(X_i,Y_i)$ where $j$'th sample is $X_{ij},Y_{ij} \in \{-1,1\}^d \times \{-1,1\}$. It is assumed that there is an underlying logistic distribution on $(X,Y)$ such that for a true parameter $\vct{\theta} \in \mathbb{R}^d$, $P(Y=y|X=\bx) = 1 /(1+\exp(-y\langle \vct{\theta}, \bx \rangle))$. Note in the classical logistic regression problem the goal is to minimize the negative log likelihood, which for a given sample has the form $l(\theta,(x,y))= \log(1+\exp(-y\langle \theta, x \rangle))$. For simplicity let us omit the client index and denote sample $(X_{ij},Y_{ij})$ as $(X_j,Y_j)$. Let us consider a one-dimensional case, this loss can be easily obtained, through a maximum likelihood argument, as follows:
%\begin{align}
%	L(\theta,(X,Y)) = \prod_i^n P(Y=y_i|X=x_i) = \prod_i^n (\frac{\exp((-y_i\langle \theta_i, x_i \rangle)}{1+\exp((-y_i\langle \theta_i, x_i \rangle)})^{(\frac{y_i+1}{2})}(\frac{1}{1+\exp((-y_i\langle \theta_i, x_i \rangle)})^{(1-\frac{y_i+1}{2})}
%\end{align}
%%\cred{$y_i$'s are missing in the exponents -- $\exp(y_i\theta x_i)$ instead of $\exp(\theta x_i)$? That is how you get the equation below?}
%%
%%Hence, the log likelihood is:
%%\begin{align}
%%	l(\theta,(X,Y)) = \sum_i^n -\log(1+\exp(-y_i \theta x_i))
%%\end{align}
%%Note when $(x_iy_i)_l=1$
%%Since $x_i\in\{-1,1\}$, we can let $q_i=x_iy_i$ and rewrite the optimization problem in one data sample $q_i$. Now the likelihood function becomes:
%%
%%\begin{align}
%%	L(\theta,Q) = \prod_i^n P(Q = q_i) = \prod_i^n (\frac{\exp(\theta )}{1+\exp(\theta )})^{(\frac{q_i+1}{2})}(\frac{1}{1+\exp(\theta )})^{(1-\frac{q_i+1}{2})}
%%\end{align}
%%\cred{I don't understand how we got this?}
%
%\textbf{Connecting to Bernoulli Setting.} Similar to \cite{duchi2019lower}, let prior probability $P(Y=y)=\frac{1}{2}$; then by construction we have $X^{l}Y\sim \Bern(p=e^\theta/(1+e^\theta))$ for any coordinate $l$, independent of others \cite{duchi2019lower}. This allow us to reduce the dataset to a single variable $Q^l=X^lY$. As a result, to find optimal $\theta_i$ we can consider the logistic regression problem separately for each coordinate, at each client $i$:
%\begin{align}
%	L^{l}(\theta,(X,Y)) = \prod_i^n P(Y=y_i|X^l=x_i) = \prod_i^n (\frac{\exp((-y_i\theta^{l}_i x^{l}_i )}{1+\exp((-y_i\theta^{l}_i x^{l}_i )})^{(\frac{y_i+1}{2})}(\frac{1}{1+\exp((-y_i\theta^{l}_i x^{l}_i )})^{(1-\frac{y_i+1}{2})}
%\end{align}
%
%Defining $q_i^l = y_ix_i^l$ this is equivalent to the following problem: 
%
%\begin{align*}
%	L^{l}(\theta_i,Q_i) = \prod_j^n P(Q_i = q_i) &= \prod_j^n (\frac{\exp(\theta_i )}{1+\exp(\theta_i )})^{(\frac{q_j+1}{2})}(\frac{1}{1+\exp(\theta_i )})^{(1-\frac{q_j+1}{2})} \\
%	&= \prod_j^n (p_i)^{(\frac{q_j+1}{2})}(1-p_i)^{(1-\frac{q_j+1}{2})} 
%\end{align*}
%\cred{In the above set of equations, it looks like indices $i$ and $j$ are not proper...}
%
%In other words for any client, finding $p_i$ and $\theta_i$ are equivalent problems. And the problem is the same as the local estimation problem that we posed before. Consequently, we can personalize the problem by employing prior of the parameter $p_i$. Assuming a Beta prior with known parameters $\alpha, \beta$:
%
%\begin{align}
%	L^{(p)}(\theta_i,Q_i) = \prod_j^n \left( p_i^{(\frac{q_j+1}{2})}(1-p_i)^{(1-\frac{q_j+1}{2})}\frac{1}{B(\alpha,\beta)} p_i^{\alpha-1} (1-p_i)^{\beta-1} \right)
%\end{align}
%
%Then the negative log likelihood becomes:
%\begin{align*}
%	l^{(p)}(\theta_i,Q_i) &= -\sum_j^n \left[{(\frac{q_j+1}{2})}\log(p_i)+{(1-\frac{q_j+1}{2})}\log(1-p_i) + (\alpha-1)\log(p_i) +(\beta-1)\log (1-p_i) \right] \\ 
%	&\hspace{5cm} \cred{+ n\log(B(\alpha,\beta))}\\
%	&= \sum_j^n \left[ \log(1+e^{-q_j\theta_i}) +  (\alpha-1)\log(1+e^{-\theta_i}) +(\beta-1)\log (1+e^{\theta_i}) \right] 
%\end{align*}
%\cred{How did we get the 2nd equality above?}
%
%Classical way of finding the minimizer in logistic regression problem is gradient descent, let us observe how our prior affects the gradient step. Taking the derivative of negative log likelihood function with respect to $\theta_i$ we have \cred{(the following does not seem to be correct: summation is missing as well as the negative signs in the exponents)}:
%\begin{align*}
%	\frac{\partial l^{(p)}(\theta_i,Q_i)}{\partial \theta_i} = -\frac{q_i}{1+e^{q_i\theta_i}} -  (\alpha-1) \frac{1}{1+e^{\theta_i}} +  (\beta-1)\frac{1}{1+e^{-\theta_i}}  
%\end{align*}
%
%Beta distribution represents a prior knowledge/experience in the form of observing past Bernoulli trials. If the ratio $\alpha/\beta$ is large you believe $p_i$ should be close to 1 and vice versa. The absolute values of $\alpha$ and $\beta$ are also important, the larger these values the more your confidence in your prior beliefs. If $\alpha$ and $\beta$ are small regardless of the ratio you will not rely on the prior information much. This effect can be better understood looking at mean and variance of $Beta$ distribution. In particular, variance decreases with the increased $\alpha, \beta$, and, mean depends solely on the ratio $\alpha/\beta$. In this paper, we characterize the heterogeneity with the variance of the global distribution, in this section our observation still holds: lower global variance, i.e. lower heterogeneity in the system, means you should benefit from global distribution more. Moreover, the gradient update can be seen as an update towards the mode of posterior distribution.\\




==> app_learn_logistic_DD.tex <==
%As described in Section~\ref{sec:learning}, by taking $\bbP(\Gamma)\equiv\calN(\vct{\mu},\sigmatheta^2\bbI_d)$ and $p_{\theta_i}(Y_{ij}|X_{ij})=\sigma(\langle \vct{\theta}_i, X_{ij} \rangle)^{Y_{ij}}(1-\sigma(\langle \vct{\theta}_i, X_{ij} \rangle))^{(1-Y_{ij})}$, where $\sigma(z)=\nicefrac{1}{1+e^{-z}}$ for any $z\in\bbR$, then the overall optimization problem becomes:
%
%%$f_i(\vct{\theta}_i)$ is the cross-entropy loss (or the logistic loss) as in the case of logistic regression.
%%
%%Now we write down the full objective function for linear regression by taking $\bbP(\Gamma)\equiv\calN(\vct{\mu},\sigmatheta^2\bbI_d)$ and $p_{\theta_i}(Y_{ij}|X_{ij})$ according to $\calN(\vct{\theta}_i,\sigma_x^2)$; the case of logistic regression can be similarly handled. Here, if we assume that in addition to $\vct{\mu}$, the other parameters $\sigmatheta,\sigma_x$ are also unknown, then we can also optimize over them. In this case, the overall optimization problem becomes:
%\begin{align}\label{eqn:logistic-regression}
%&\argmin_{\{\vct{\theta}_i\},\vct{\mu}, \sigmatheta}\sum_{i=1}^{m}\sum_{j=1}^{n}\left[Y_{ij}\log\left(\frac{1}{1+e^{-\langle\vct{\theta}_i,X_{ij}\rangle}}\right) + (1-Y_{ij})\log\left(\frac{1}{1+e^{\langle\vct{\theta}_i,X_{ij}\rangle}}\right)\right] \notag \\
%&\hspace{5cm} +\frac{md}{2}\log(2\pi\sigma_{\theta}^2)+\sum_{i=1}^{m}\frac{\|\vct{\mu}-\vct{\theta}_i\|_2^2}{2\sigma_{\theta}^2}.
%\end{align}
%
%%\textbf{General Logistic Regression Setting.} Considering a general cases/datasets, it is useful to derive the prior as a generating model for $\vct{\theta}$. In particular, as in linear regression case, if we assume $\vct{\theta}_i \sim N(\vct{\mu}, \sigma_{\theta}^2\mathbb{I}_{dxd})$ we obtain the following MAP problem:  
%%
%%\begin{align*}
%%	\hat{\vct{\theta}}_1,\ldots,\hat{\vct{\theta}}_m &= \argmax f_{\theta|\mathbf{X},\mathbf{Y}}\\
%%	&= \argmin  \sum_{i=1}^m \sum_{j=1}^n \left( (y_j)\log\left(\frac{1}{1+e^{-\vct{\theta}_i^Tx_j}}\right)+(1-y_j)\log\left(\frac{1}{1+e^{\vct{\theta}_i^Tx_j}}\right) \right) \\
%%	& \quad +\frac{md}{2}\log(2\pi\sigma_{\theta}^2)+\sum_{i=1}^{m}\frac{\|\vct{\mu}-\vct{\theta}_i\|^2}{2\sigma_{\theta}^2}.
%%\end{align*}
%
%When $\vct{\mu}$ and $\sigma_{\theta}^2$ are unknown, we would like to learn them by gradient descent, as in the linear regression case. The corresponding algorithm is described in Algorithm~\ref{algo:personalized_logsitic_regression}.
%
%\begin{algorithm}[H]
%	\caption{Logistic Regression SGD}
%	{\bf Input:} Number of iterations $T$, local datasets $(Y_i, X_i)$ for $i\in[m]$, learning rate $\eta$.\\
%	\vspace{-0.3cm}
%	\begin{algorithmic}[1] 	\label{algo:personalized_logsitic_regression}
%		\STATE \textbf{Initialize} $\vct{\theta}_i^{0}$  for $i\in[m]$, $\vct{\mu}^0$, $\sigma_{\theta}^{2,0}$.
%		\FOR{$t=1$ \textbf{to} $T$} 
%		\STATE \textbf{On Clients:}
%		\FOR {$i=1$ \textbf{to} $m$:}
%		\STATE Receive $(\vct{\mu}^{t},\sigma^{2,t}_{\theta})$ from the server and set $\vct{\mu}_{i}^t := \vct{\mu}^{t},\sigma^{2,t}_{\theta,i}:=\sigma^{2,t}_{\theta}$
%		\STATE Update the personalized model: \[\vct{\theta}_i^{t}\gets\vct{\theta}_{i}^{t-1}-\eta\left(\sum_{j=1}^{n}\nabla_{\theta_i^{t-1}}l_{CE}^{(p)}(\vct{\theta}_i^{t-1}, (X_i^j,Y_i^j))+\frac{\vct{\mu}_i^{t-1}-\vct{\theta}_i^{t-1}}{\sigma_{\theta,i}^{2,t-1}}\right),\]
%		where $l_{CE}^{(p)}$ denotes the cross-entropy loss.
%		\STATE Update local version of mean: $\vct{\mu}_i^{t}\gets\vct{\mu}_i^{t-1}-\eta\left(\frac{\vct{\mu}_i^{t-1}-\vct{\theta}_i^{t-1}}{\sigma_{\theta,_i}^{2,t-1}}\right)$
%		\STATE Update global variance: $\sigma^{2,t}_{\theta,_i}\gets\sigma^{2,t-1}_{\theta,_i}-\eta\left(\frac{d}{2\sigma_{\theta,i}^{2,t-1}}-\frac{\|\vct{\mu}_i^{t-1}-\vct{\theta}^{t-1}_i\|^2}{2(\sigma_{\theta,i}^{2,t-1})^2}\right)$
%		\STATE Send $(\vct{\mu}_i^t,\sigma_{\theta,i}^{2,t})$ to the server
%		\ENDFOR
%		\STATE \textbf{At the Server:}
%		\STATE Receive $\{(\vct{\mu}_i^t,\sigma_{\theta,i}^{2,t})\}$ from the clients
%		\STATE Aggregate mean: $\vct{\mu}^{t}=\frac{1}{m}\sum_{i=1}^{m}\vct{\mu}_i^t$
%		\STATE Aggregate global variance: $\sigma^{2,t}_{\theta}= \frac{1}{m}\sum_{i=1}^{m}\sigma^{2,t}_{\theta,i}$
%		\STATE Broadcast $(\vct{\mu}^{t},\sigma^{2,t}_{\theta})$ to all clients
%		\ENDFOR
%	\end{algorithmic}
%	{\bf Output:} Personalized models $\vct{\theta}_1^{T},\ldots,\vct{\theta}_m^{T}$.
%\end{algorithm}

\iffalse
\textbf{A simplified version that connects to the Bernoulli model.} An interesting observation can be made when we examine a simplified version of logistic regression which is considered in \cite{duchi2019lower}. Consider a simplified logistic regression problem as in \cite{duchi2019lower}, where a client $i$ possesses local dataset tuple $(X_i,Y_i)$ where $j$'th sample is $X_{ij},Y_{ij} \in \{-1,1\}^d \times \{-1,1\}$. It is assumed that there is an underlying logistic distribution on $(X,Y)$ such that for a true parameter $\vct{\theta} \in \mathbb{R}^d$, $P(Y=y|X=\bx) = 1 /(1+\exp(-y\langle \vct{\theta}, \bx \rangle))$. Note in the classical logistic regression problem the goal is to minimize the negative log likelihood, which for a given sample has the form $l(\vct{\theta},(x,y))= \log(1+\exp(-y\langle \vct{\theta}, x \rangle))$. For simplicity let us omit the client index and denote sample $(X_{ij},Y_{ij})$ as $(X_j,Y_j)$. Let us consider a one-dimensional case, this loss can be easily obtained, through a maximum likelihood argument, as follows:
\begin{align}
	L(\vct{\theta},(X,Y)) = \prod_i^n P(Y=y_i|X=x_i) = \prod_i^n (\frac{\exp((-y_i\langle \vct{\theta}_i, x_i \rangle)}{1+\exp((-y_i\langle \vct{\theta}_i, x_i \rangle)})^{(\frac{y_i+1}{2})}(\frac{1}{1+\exp((-y_i\langle \vct{\theta}_i, x_i \rangle)})^{(1-\frac{y_i+1}{2})}
\end{align}
%\cred{$y_i$'s are missing in the exponents -- $\exp(y_i\vct{\theta} x_i)$ instead of $\exp(\vct{\theta} x_i)$? That is how you get the equation below?}
%
%Hence, the log likelihood is:
%\begin{align}
%	l(\vct{\theta},(X,Y)) = \sum_i^n -\log(1+\exp(-y_i \vct{\theta} x_i))
%\end{align}

Since $x_i\in\{-1,1\}$, we can let $q_i=x_iy_i$ and rewrite the optimization problem in one data sample $q_i$. Now the likelihood function becomes:

\begin{align}
	L(\vct{\theta},Q) = \prod_i^n P(Q = q_i) = \prod_i^n (\frac{\exp(\vct{\theta} )}{1+\exp(\vct{\theta} )})^{(\frac{q_i+1}{2})}(\frac{1}{1+\exp(\vct{\theta} )})^{(1-\frac{q_i+1}{2})}
\end{align}
\cred{I don't understand how we got this?}

\textbf{Connecting to Bernoulli Setting.} Similar to \cite{duchi2019lower}, let prior probability $P(Y=y)=\frac{1}{2}$; then by construction we have $XY\sim \Bern(p=e^\vct{\theta}/(1+e^\vct{\theta}))$. As a result, for client $i$:

\begin{align*}
	L(\vct{\theta}_i,Q_i) = \prod_j^n P(Q_i = q_i) &= \prod_j^n (\frac{\exp(\vct{\theta}_i )}{1+\exp(\vct{\theta}_i )})^{(\frac{q_j+1}{2})}(\frac{1}{1+\exp(\vct{\theta}_i )})^{(1-\frac{q_j+1}{2})} \\
	&= \prod_j^n (p_i)^{(\frac{q_j+1}{2})}(1-p_i)^{(1-\frac{q_j+1}{2})} 
\end{align*}
\cred{In the above set of equations, it looks like indices $i$ and $j$ are not proper...}

In other words for any client, finding $p_i$ and $\vct{\theta}_i$ are equivalent problems. And the problem is the same as the local estimation problem that we posed before. Consequently, we can personalize the problem by employing prior of the parameter $p_i$. Assuming a Beta prior with known parameters $\alpha, \beta$:

\begin{align}
	L^{(p)}(\vct{\theta}_i,Q_i) = \prod_j^n \left( p_i^{(\frac{q_j+1}{2})}(1-p_i)^{(1-\frac{q_j+1}{2})}\frac{1}{B(\alpha,\beta)} p_i^{\alpha-1} (1-p_i)^{\beta-1} \right)
\end{align}

Then the negative log likelihood becomes:
\begin{align*}
	l^{(p)}(\vct{\theta}_i,Q_i) &= -\sum_j^n \left[{(\frac{q_j+1}{2})}\log(p_i)+{(1-\frac{q_j+1}{2})}\log(1-p_i) + (\alpha-1)\log(p_i) +(\beta-1)\log (1-p_i) \right] \\ 
	&\hspace{5cm} \cred{+ n\log(B(\alpha,\beta))}\\
	&= \sum_j^n \left[ \log(1+e^{-q_j\vct{\theta}_i}) +  (\alpha-1)\log(1+e^{-\vct{\theta}_i}) +(\beta-1)\log (1+e^{\vct{\theta}_i}) \right] 
\end{align*}
\cred{How did we get the 2nd equality above?}

Classical way of finding the minimizer in logistic regression problem is gradient descent, let us observe how our prior affects the gradient step. Taking the derivative of negative log likelihood function with respect to $\vct{\theta}_i$ we have \cred{(the following does not seem to be correct: summation is missing as well as the negative signs in the exponents)}:
\begin{align*}
	\frac{\partial l^{(p)}(\vct{\theta}_i,Q_i)}{\partial \vct{\theta}_i} = -\frac{q_i}{1+e^{q_i\vct{\theta}_i}} -  (\alpha-1) \frac{1}{1+e^{\vct{\theta}_i}} +  (\beta-1)\frac{1}{1+e^{-\vct{\theta}_i}}  
\end{align*}

Beta distribution represents a prior knowledge/experience in the form of observing past Bernoulli trials. If the ratio $\alpha/\beta$ is large you believe $p_i$ should be close to 1 and vice versa. The absolute values of $\alpha$ and $\beta$ are also important, the larger these values the more your confidence in your prior beliefs. If $\alpha$ and $\beta$ are small regardless of the ratio you will not rely on the prior information much. This effect can be better understood looking at mean and variance of $Beta$ distribution. In particular, variance decreases with the increased $\alpha, \beta$, and, mean depends solely on the ratio $\alpha/\beta$. In this paper, we characterize the heterogeneity with the variance of the global distribution, in this section our observation still holds: lower global variance, i.e. lower heterogeneity in the system, means you should benefit from global distribution more. Moreover, the gradient update can be seen as an update towards the mode of posterior distribution.\\
\fi



==> app_learn_mixture.tex <==
%\cred{This is about Linear Regression with Discrete prior...}
In this section, we present the linear regression problem as a generalization to the estimation problem with discrete priors.


Consider A set of $m$ clients, where the $i$-th client has a local dataset $(y_{i1},x_{i1}),\ldots,(y_{in},x_{in})$ of $m$ samples, where $x_{ij}\in\mathbb{R}^{d}$ denotes the feature vector and $y_{ij}\in\mathbb{R}$ denotes the corresponding response. Let $Y_i=(y_{i1},\ldots,y_{i1})\in\mathbb{R}^{n}$ and $X_i=(x_{i1},\ldots,x_{in})\in\mathbb{R}^{n\times d}$ denote the response vector and the feature matrix at the $i$-th client, respectively. Following the standard regression, we assume that the response vector $Y_i$ is obtained from a linear model as follows:
\begin{equation}\label{linear_reg}
Y_i = X_i \theta_i+w_i,    
\end{equation}
where $\theta_i$ denotes personalized model of the $i$-th client and $w_i\sim\mathcal{N}\left(0,\sigma_x^2\mathbb{I}_{n\times n}\right)$ is a noise vector. The clients models are drawn i.i.d. from a discrete distribution $\theta_1,\ldots,\theta_{m}\sim P$, where $P=[p_1,\ldots,p_k]$ such that $p_l=\Pr[\theta_i=\mu_l]$ for $i\in[m]$ and $l\in[k]$. Our goal is to minimize the mean squared error (MSE) of each client:
\begin{equation}
    MSE = \mathbb{E}_{\lbrace w_l,\theta_l\rbrace}\left[\|Y_i-X_i\theta_i\|^2\right],
\end{equation}
where the expectation is taken with respect to the random noise and the local models $\theta_1,\ldots,\theta_m$. We assume that the discrete distribution $P$ and the prior candidates $\lbrace \mu_l \rbrace_{l=1}^{k}$ are unknown to the clients. Inspired from Algorithm~\ref{algo:cluster}
for estimation with discrete priors, we obtain Algorithm~\ref{algo:cluster_linear_regression}, where we initialize the personalized models $\theta_i^{(0)}=(X_i^{T}X_i)^{-1}X_i^{T}Y_i$ which is the optimal model as a function of the local dataset without any prior knowledge. Furthermore, for given the prior information $P^{(t)}$, $\lbrace \mu_l^{(t)}\rbrace$, the $i$-th client updates the personalized model as $\theta_i^{t}= \sum_{l=1}^{k}\alpha_{l}^{(i)}\mu_l^{(t)}$, where the weights $\alpha_{l}^{(i)}\propto p_l^{(t)}\exp\left(-\frac{\|X_i\mu_l^{(t)}-Y_i\|^2}{2\sigma_x^2}\right)$ that decreases when the loss function $\|X_i\mu_l^{(t)}-Y_i\|^2$ increases and/or the prior distribution $p_l^{(t)}$ decreases. Note that this is \emph{not} a new algorithm, and is essentially the algorithm proposed in \cite{marfoq2021federated} applied to \eqref{linear_reg}. We wanted to show how our framework captures mixture model in \cite{marfoq2021federated} through this example.



\begin{algorithm}[H]
			\caption{Alternating Minimization Estimation}
			{\bf Input:} Number of iterations $T$, local datasets $(Y_i,X_i)$ for $i\in[m]$.\\
			\vspace{-0.3cm}
			\begin{algorithmic}[1] 	\label{algo:cluster_linear_regression}
			\STATE \textbf{Initialize} $\theta_i^{0}=(X_i^{T}X_i)^{-1}X_i^{T}Y_i$  for $i\in[m]$.
			\FOR{$t=1$ \textbf{to} $T$}
			\STATE~\label{step:clustering} \textbf{Update the priors:}
			$P^{(t)},\mu_1^{(t)},\ldots,\mu_k^{(t)}\gets \mathsf{Cluster}\left(\theta_1^{(t-1)},\ldots,\theta_m^{(t-1)},k\right)$
			\FOR {$i=1$ \textbf{to} $m$:}
			\STATE ~\label{step:personal_update} \textbf{Update the personalized model:} $\theta_i^{t}\gets \sum_{l=1}^{k}\alpha_{l}^{(i)}\mu_l^{(t)}$ and $\alpha_{l}^{(i)}=\frac{p_l^{(t)}\exp{-\frac{\|X_{i}\mu_l^{(t)}-Y_i\|^2}{2\sigma_x^2}}}{\sum_{s=1}^{k}p_s^{(t)}\exp{-\frac{\|X_{i}\mu_s^{(t)}-Y_i\|^2}{2\sigma_x^2}}}$
			\ENDFOR
			\ENDFOR
			\end{algorithmic}
			{\bf Output:} Personalized models $\theta_1^{T},\ldots,\theta_m^{T}$.
\end{algorithm}




==> app_learn_mixture_DD.tex <==
%\cred{This is about Linear Regression with Discrete prior...}
%In this section, we present the linear regression problem as a generalization to the estimation problem with discrete priors. This model falls into the framework studied in \cite{marfoq2021federated} and is illustrated to show how our framework also captures it.
%
%
%Consider a set of $m$ clients, where the $i$-th client has a local dataset $(X_{i1},Y_{i1}),\ldots,(X_{in},Y_{in})$ of $m$ samples, where $X_{ij}\in\mathbb{R}^{d}$ denotes the feature vector and $Y_{ij}\in\mathbb{R}$ denotes the corresponding response. Let $Y_i=(Y_{i1},\ldots,Y_{i1})\in\mathbb{R}^{n}$ and $X_i=(X_{i1},\ldots,X_{in})\in\mathbb{R}^{n\times d}$ denote the response vector and the feature matrix at the $i$-th client, respectively. Following the standard regression, we assume that the response vector $Y_i$ is obtained from a linear model as follows:
%\begin{equation}
%Y_i = X_i \vct{\theta}_i+\bw_i,    
%\end{equation}
%where $\vct{\theta}_i$ denotes personalized model of the $i$-th client and $\bw_i\sim\mathcal{N}\left(0,\sigma_x^2\mathbb{I}_{n}\right)$ is a noise vector. The clients models are drawn i.i.d. from a discrete distribution $\vct{\theta}_1,\ldots,\vct{\theta}_{m}\sim \bbP$, where $\bbP=[p_1,\ldots,p_k]$ such that $p_l=\Pr[\vct{\theta}_i=\vct{\mu}_l]$ for $i\in[m]$ and $l\in[k]$. 
%
%%Our goal is to minimize the mean squared error (MSE) of each client:
%%\begin{equation}
%%    MSE = \mathbb{E}_{\lbrace w_l,\vct{\theta}_l\rbrace}\left[\|Y_i-X_i\vct{\theta}_i\|^2\right],
%%\end{equation}
%%where the expectation is taken with respect to the random noise and the local models $\vct{\theta}_1,\ldots,\vct{\theta}_m$. 
%
%Our goal is to solve the optimization problem stated in \eqref{eq:learning-log-generative-model} (for the linear regression with the above discrete prior) and learn the optimal personalized parameters $\{\htheta_i\}$.
%
%We assume that the discrete distribution $\bbP$ and the prior candidates $\lbrace \vct{\mu}_l \rbrace_{l=1}^{k}$ are unknown to the clients. Inspired from Algorithm~\ref{algo:cluster} for estimation with discrete priors, we obtain Algorithm~\ref{algo:cluster_linear_regression} for learning with discrete prior. 
%Note that this is \emph{not} a new algorithm, and is essentially the algorithm proposed in \cite{marfoq2021federated} applied to linear regression. We wanted to show how our framework captures mixture model in \cite{marfoq2021federated} through this example.
%%This will exactly lead to the discrete mixture framework \citep{marfoq2021federated}, specialized to the linear regression model.
%
%\textbf{Description of Algorithm~\ref{algo:cluster_linear_regression}.} Client $i$ initializes its personalized parameters $\vct{\theta}_i^{(0)}=(X_i^{T}X_i)^{-1}X_i^{T}Y_i$, which is the optimal as a function of the local dataset at the $i$-th client without any prior knowledge. 
%In any iteration $t$, for a given prior information $\bbP^{(t)}$, $\lbrace \vct{\mu}_l^{(t)}\rbrace$, the $i$-th client updates the personalized model as $\vct{\theta}_i^{t}= \sum_{l=1}^{k}\alpha_{l}^{(i)}\vct{\mu}_l^{(t)}$, where the weights $\alpha_{l}^{(i)}\propto p_l^{(t)}\exp\left(-\frac{\|X_i\vct{\mu}_l^{(t)}-Y_i\|^2}{2\sigma_x^2}\right)$ and sends its current estimate of the personalized parameter $\vct{\theta}_i^t$ to the server. Upon receiving $\vct{\theta}_1^t,\ldots,\vct{\theta}_m^t$, server will run $\mathsf{Cluster}$ algorithm to update the global parameters $\bbP,\vct{\mu}_1^{(t)},\ldots,\vct{\mu}_k^{(t)}$, and broadcasts them to the clients. 
%%The full algorithm is presented in Algorithm~\ref{algo:cluster_linear_regression}.
%
%
%
%
%\begin{algorithm}[h]
%			\caption{Alternating Minimization for Personalized Learning}
%			{\bf Input:} Number of iterations $T$, local datasets $(X_i,Y_i)$ for $i\in[m]$.\\
%			\vspace{-0.3cm}
%			\begin{algorithmic}[1] 	\label{algo:cluster_linear_regression}
%			\STATE \textbf{Initialize} $\vct{\theta}_i^{0}=(X_i^{T}X_i)^{-1}X_i^{T}Y_i$  for $i\in[m]$ (if $X_i^{T}X_i$ is not full-rank, take the pseudo-inverse).
%			\FOR{$t=1$ \textbf{to} $T$}
%			\STATE {\bf On Clients:}
%			\FOR {$i=1$ \textbf{to} $m$:}
%			\STATE Receive $\bbP^{(t)},\vct{\mu}_1^{(t)},\ldots,\vct{\mu}_k^{(t)}$ from the server 
%			\STATE\label{step:personal_update} Update the personalized parameters and the coefficients:
%			\begin{align*}
%			\vct{\theta}_i^{t} \gets \sum_{l=1}^{k}\alpha_{l}^{(i)}\vct{\mu}_l^{(t)} \qquad \text{ and } \qquad
%			\alpha_{l}^{(i)} =\frac{p_l^{(t)}\exp\left(-\frac{\|X_{i}\vct{\mu}_l^{(t)}-Y_i\|^2}{2\sigma_x^2}\right)}{\sum_{s=1}^{k}p_s^{(t)}\exp\left(-\frac{\|X_{i}\vct{\mu}_s^{(t)}-Y_i\|^2}{2\sigma_x^2}\right)}
%			\end{align*}
%			\STATE Send $\vct{\theta}_i^{(t)}$ to the server
%			\ENDFOR
%			\STATE {\bf At the Server:}
%			\STATE Receive $\vct{\theta}_1^{(t)},\ldots,\vct{\theta}_m^{(t)}$ from the clients
%			\STATE\label{step:clustering} Update the global parameters:
%			$\bbP^{(t)},\vct{\mu}_1^{(t)},\ldots,\vct{\mu}_k^{(t)}\gets \mathsf{Cluster}\left(\vct{\theta}_1^{(t)},\ldots,\vct{\theta}_m^{(t)},k\right)$
%			\STATE Broadcast $\bbP^{(t)},\vct{\mu}_1^{(t)},\ldots,\vct{\mu}_k^{(t)}$ to all clients
%			\ENDFOR
%			\end{algorithmic}
%			{\bf Output:} Personalized models $\vct{\theta}_1^{T},\ldots,\vct{\theta}_m^{T}$.
%\end{algorithm}




==> app_soc_impact_limitations.tex <==
%\subsection{Societal Impact and Limitations}
%
%\textbf{Societal Impact.} In this work we consider learning through
%collaboration of many users. Hence, a potential societal impact is on
%users' privacy. For instance, clustering/mixture based methods can
%breach the users' privacy; or shared models can introduce privacy
%leaks. To ameliorate this, we propose differential privacy techniques
%that helps to preserve users' privacy. In our setting, we consider
%collaboration of diverse clients which may potentially have a positive
%impact on society. As we have seen collaborative personalization, can
%significantly improve learning performance. However, such
%personalization is only as good as the data used for training, and if
%not used properly could lead to information bubbles and disjointed
%views for each client. These could be accentuated with clustering
%methods that put together clients with similar data statistics, and
%therefore such methods need to be used properly. However, our approach
%does not restrict it such global models and can fine-tune the local
%models iteratively to obtain better performance and potentially reduce
%this effect. However, there is still a lot of work to be addressed,
%including fairness across users; a topic for future work.
%
%
%%This paper considers collaborative personalization in learning, which
%%can significantly improve learning performance. However, such
%%personalization is only as good as the data used for training, and if
%%not used properly could lead to information bubbles and disjointed
%%views for each client, \emph{e.g.,} clustering methods that put
%%together clients with similar data statistics. We ameliorate that by
%%not clustering similar data and models, but this is an aspect that
%%might need more examination for social consequences. We explicitly
%%consider diverse resources in our designs, potentially enabling
%%clients with fewer resources (devices with less capabilities) to
%%benefit from richer resources; potentially a positive impact in using
%%resources more equitably. 
%
%\textbf{Limitations and future work.} There are several open questions
%that remain from this work, pointing to some of its limitations.
%%One such question is to consider convergence guarantees for our algorithms such as AdaPeD.
%One question is proving information-theoretic
%lower bounds for estimation and learning under information
%constraints, such as communication or privacy; our methods provided
%schemes and achievable performances. Also we leave testing our
%algorithms in very large scale to practitioners, as such large-scale
%evaluations are perhaps more feasible with large computing and
%networking resources.


%\subsection{Preliminaries}

%definitions of CDP, LDP, RDP, composition, user-level privacy and related preliminaries needed for all the proofs

We give standard privacy definitions that we use in Section~\ref{sec:priv-defn}, some existing results on RDP to DP conversion and RDP composition in Section~\ref{sec:RDP-DP}, and user-level differential privacy in Section~\ref{sec:user-level-dp}.

\subsection{Privacy Definitions}\label{sec:priv-defn}
In this subsection, we define different privacy notions that we will use in this paper: local differential privacy (LDP), central different privacy (DP), and Renyi differential privacy (RDP), and their user-level counterparts.
\begin{definition}[Local Differential Privacy - LDP~\citep{kasiviswanathan2011can}]~\label{defn:LDPdef}
For $\epsilon_0\geq0$, a randomized mechanism $\calR:\calX\to\calY$ is said to be $\eps_0$-local differentially private (in short, $\eps_{0}$-LDP), if for every pair of inputs $d,d'\in\calX$, we have 
\begin{equation}~\label{ldp-def}
\Pr[\calR(d)\in \calS] \leq e^{\eps_0}\Pr[\calR(d')\in \calS], \qquad \forall \calS\subset\calY.
\end{equation}
\end{definition}
Let $\calD=\lbrace x_1,\ldots,x_n\rbrace$ denote a dataset comprising $n$ points from $\calX$. We say that two datasets $\calD=\lbrace x_1,\ldots,x_n\rbrace$ and $\calD^{\prime}=\lbrace x_1^{\prime},\ldots,x_n^{\prime}\rbrace$ are neighboring (and denoted by $\calD\sim\calD'$) if they differ in one data point, i.e., there exists an $i\in[n]$ such that $x_i\neq x'_i$ and for every $j\in[n],j\neq i$, we have $x_j=x'_j$.
\begin{definition}[Central Differential Privacy - DP \citep{Calibrating_DP06,dwork2014algorithmic}]\label{defn:central-DP}
For $\epsilon,\delta\geq0$, a randomized mechanism $\calM:\calX^n\to\calY$ is said to be $(\epsilon,\delta)$-differentially private (in short, $(\epsilon,\delta)$-DP), if for all neighboring datasets $\calD\sim\calD^{\prime}\in\calX^{n}$ and every subset $\calS\subseteq \calY$, we have
\begin{equation}~\label{dp_def}
\Pr\left[\calM(\calD)\in\calS\right]\leq e^{\eps_0}\Pr\left[\calM(\calD^{\prime})\in\calS\right]+\delta.
\end{equation}
If $\delta = 0$, then the privacy is referred to as pure DP.
\end{definition}

\begin{definition}[$(\lambda,\epsilon(\lambda))$-RDP (Renyi Differential Privacy)~\citep{RDP_Mironov17}]\label{defn:RDP}
A randomized mechanism $\calM:\calX^n\to\calY$ is said to have $\epsilon(\lambda)$-Renyi differential privacy of order $\lambda\in(1,\infty)$ (in short, $(\lambda,\epsilon(\lambda))$-RDP), if for any neighboring datasets $\calD\sim\calD'\in\calX^n$, the Renyi divergence between $\calM(\calD)$ and $\calM(\calD')$ is upper-bounded by $\eps(\lambda)$, i.e.,
\begin{align*}
D_{\lambda}(\calM(\calD)||\calM(\calD'))&=\frac{1}{\lambda-1}\log\left(\mathbb{E}_{\theta\sim\calM(\calD')}\left[\left(\frac{\calM(\calD)(\theta)}{\calM(\calD')(\theta)}\right)^{\lambda}\right]\right)\\
&\leq \epsilon(\lambda),
\end{align*}
where $\calM(\calD)(\theta)$ denotes the probability that $\calM$ on input $\calD$ generates the output $\theta$. For convenience, instead of $\eps(\lambda)$ being an upper bound, we define it as $\eps(\lambda)=\sup_{\calD\sim\calD'}D_{\lambda}(\calM(\calD)||\calM(\calD'))$.
\end{definition}
%
%Our objective in this paper is to characterize the Renyi differential privacy of a shuffling mechanism $\calM$ (see Section~\ref{subsec:prob-form} for details) for different values of order $\lambda$. 
%Thus, it is convenient to write the parameter $\epsilon$ of the mechanism $\calM$ as a function of $\lambda$, i.e., a mechanism $\calM$ is $(\lambda,\epsilon(\lambda))$-RDP, where $\epsilon(\lambda)$ is a function of the order $\lambda$. For convenience, instead of $\eps(\lambda)$ being an upper bound, we will define it as
%\begin{align}
%\end{align}

\subsection{RDP to DP Conversion and RDP Composition}\label{sec:RDP-DP}
%In this subsection, we state some preliminary results from the literature that we will use. Though our main objective in this paper is to derive RDP guarantees of a shuffling mechanism, we also give the central privacy guarantees of that mechanism. 
As mentioned after Theorem~\ref{thm:privacy_personal}, we can convert the RDP guarantees of \dpadaped\ to its DP guarantees using existing conversion results from literature. To the best of our knowledge, the following gives the best conversion.
%For that purpose, we use the following result for converting the RDP guarantees of a mechanism to its DP guarantees. To the best of our knowledge, this result gives the best conversion. %\footnote{An optimal conversion from RDP to approximate DP was studied in \citep{asoodeh2021three}; however, we observed numerically, that it does not give better performance as compared to the conversion presented above.} 
  %, numerical stability issues could cause some problems. An open question is how to use this optimal  conversion in a better manner.} 
\begin{lemma}[From RDP to DP~\citep{canonne2020discrete,Borja_HypTest-RDP20}]\label{lem:RDP_DP} 
Suppose for any $\lambda>1$, a mechanism $\calM$ is $\left(\lambda,\epsilon\left(\lambda\right)\right)$-RDP. Then, the mechanism $\calM$ is $\left(\epsilon,\delta\right)$-DP, where $\epsilon,\delta$ are define below: 
\begin{equation*}
\begin{aligned}
&\text{For a given }\delta\in(0,1) :\\
 & \epsilon = \min_{\lambda} \epsilon\left(\lambda\right)+\frac{\log\left(1/\delta\right)+\left(\lambda-1\right)\log\left(1-1/\lambda\right)-\log\left(\lambda\right)}{\lambda-1}\\
&\text{For a given }\epsilon>0 : \\
& \delta = \min_{\lambda}\frac{\exp\left(\left(\lambda-1\right)\left(\epsilon\left(\lambda\right)-\epsilon\right)\right)}{\lambda-1}\left(1-\frac{1}{\lambda}\right)^{\lambda}. 
\end{aligned}
\end{equation*}
\end{lemma}
%
The main strength of RDP in comparison to other privacy notions comes from composition. The following result states that if we adaptively compose two RDP mechanisms with the same order, their privacy parameters add up in the resulting mechanism.
\begin{lemma}[Adaptive composition of RDP~{\citep[Proposition~1]{RDP_Mironov17}}]\label{lemm:compostion_rdp} 
For any $\lambda>1$, let $\calM_1:\calX\to \calY_1$ be a $(\lambda,\epsilon_1(\lambda))$-RDP mechanism and $\calM_2:\calY_1\times \calX\to \calY$ be a $(\lambda,\epsilon_2(\lambda))$-RDP mechanism. Then, the mechanism defined by $(\calM_1,\calM_2)$ satisfies $(\lambda,\epsilon_1(\lambda)+\epsilon_2(\lambda))$-RDP. 
\end{lemma}
%
\iffalse
By combining the above two lemmas, we can give the DP privacy guarantee of a sequence of $T$ adaptive RDP mechanisms. Let $\calM_1\left(\calI_1,\calD\right),\ldots,\calM_T\left(\calI_T,\calD\right)$ be a sequence of $T$ adaptive mechanisms, where $\calI_t$ denotes the auxiliary input to the $t$'th mechanism, which may depend on the previous mechanisms' outputs and the auxiliary inputs $\{(\calI_i,\calM_i(\calI_i,\calD)):i<t\}$, and the $t$'th mechanism $\calM_t$ is $\left(\lambda,\epsilon_t\left(\lambda\right)\right)$-RDP. Thus, from Lemma~\ref{lemm:compostion_rdp}, we get that the mechanism defined by $\left(\calM_1,\ldots,M_T\right)$ is $\left(\lambda,\sum_{t=1}^{T}\epsilon_t\left(\lambda\right)\right)$-RDP, and then from Lemma~\ref{lem:RDP_DP} that the mechanism $\left(\calM_1,\ldots,M_T\right)$ satisfies $\left(\epsilon,\delta\right)$-DP, where $\epsilon,\delta$ are given below: 
\begin{equation*}
\begin{aligned}
&\text{For a given }\delta\in(0,1) :\\ 
&\epsilon = \min_{\lambda} \sum_{t=1}^{T}\epsilon_t\left(\lambda\right)+\frac{\log\left(1/\delta\right)+\left(\lambda-1\right)\log\left(1-1/\lambda\right)-\log\left(\lambda\right)}{\lambda-1}\\
&\text{For a given }\epsilon>0 : \\
& \delta = \min_{\lambda}\frac{\exp\left(\left(\lambda-1\right)\left(\sum_{t=1}^{T}\epsilon_t\left(\lambda\right)-\epsilon\right)\right)}{\lambda-1}\left(1-\frac{1}{\lambda}\right)^{\lambda}. 
\end{aligned}
\end{equation*} 
\fi

\subsection{User-level Differential Privacy~\cite{levy_user-level-dp21}}\label{sec:user-level-dp}
Consider a set of $m$ users, each having a local dataset of $n$ samples. Let $\calD_i=\lbrace x_{i1},\ldots,x_{in}\rbrace$ denote the local dataset at the $i$-th user for $i\in[m]$, where $x_{ij}\in\calX$ and $\calX\subset \mathbb{R}^d$. We define $\calD=(\calD_1,\ldots,\calD_{m})\in(\calX^n)^m$ as the entire dataset. %The users are connected to an untrusted server who wants to estimate the mean $\overline{x}=\frac{1}{m n}\sum_{i=1}^{n}\sum_{j=1}^{m}x_{j}^{(i)}$. Users want to preserve the privacy of their local datasets while minimizing the worst-case expected error for estimating $\overline{x}$; see \eqref{worst-case-error}.

%We first define differential privacy (DP) and the difference between user-level and item-level privacy. We say that two datasets $\calD$, $\calD'$ are neighboring with respect to distance metric $\mathsf{dis}$ if we have $\mathsf{dis}(\calD,\calD')\leq 1$. 

We have already defined DP, LDP, and RDP in Section~\ref{sec:priv-defn} w.r.t.\ the item-level privacy. Here, we extend those definition w.r.t.\ the user-level privacy. In order to do that, we need a generic neighborhood relation between datasets: We say that two datasets $\calD$, $\calD'$ are neighboring with respect to distance metric $\mathsf{dis}$ if we have $\mathsf{dis}(\calD,\calD')\leq 1$. 

%\begin{definition}(Differential Privacy)\label{defn:DP} Let $\epsilon,\delta\geq 0$. A randomized mechanism $\mathsf{M}:\calD\to\Theta$ is said to be $\left(\epsilon,\delta\right)$-DP with respect to $\mathsf{dis}$ if for any neighboring datasets $\calD,\calD'$ and any measurable set $\theta\subseteq \Theta$, we have
%\begin{equation}
%\Pr\left(\mathsf{M}\left(\calD\right)\in \theta\right)\leq e^{\epsilon}\Pr\left(\mathsf{M}\left(\calD'\right)\in \theta\right)+\delta.
%\end{equation}
%\end{definition}
%If $\delta = 0$, then the privacy is referred to as pure DP.
\textbf{Item-level DP/RDP vs.\ User-level DP/RDP.}
%When we have more than one user (i.e., $m>1$) and a space $\calD:=(\calX^{n})^m$, by 
By choosing $\mathsf{dis}(\calD,\calD')=\sum_{i=1}^{m}\sum_{j=1}^{n}\mathbbm{1}\lbrace x_{ij}\neq x_{ij}' \rbrace$, we recover the standard definition of the DP/RDP from Definitions~\ref{defn:central-DP},~\ref{defn:RDP}, which we call {\em item-level} DP/RDP. In the item-level DP/RDP, two datasets $\calD$, $\calD'$ are neighboring if they differ in a single item. On the other hand, by choosing $\mathsf{dis}(\calD,\calD')=\sum_{i=1}^{m}\mathbbm{1}\lbrace \calD_i\neq \calD'_i \rbrace$, we call it \textit{user-level} DP/RDP, where two datasets $\calD,\calD'\in (\calX^{n})^m$ are neighboring when they differ in a local dataset of any single user. Observe that when each user has a single item ($n=1$), then both item-level and user-level privacy are equivalent.   
%\end{remark}

%\begin{remark}[User-level Local Differential Privacy (LDP)] 
\textbf{User-level Local Differential Privacy (LDP).}
When we have a single user (i.e., $m=1$ and $\mathbb{\calD}=\calX^{n}$), by choosing $\mathsf{dis}\left(\calD,\calD'\right)=\mathbbm{1}\lbrace \calD\neq \calD' \rbrace$ for $\calD,\calD'\in\calX^n$, we call it \textit{user-level LDP}. In this case each user privatize her own local dataset using a private mechanism.
%\end{remark}

We can define user-level LDP/DP/RDP analogously to their item-level counterparts using the neighborhood relation $\mathsf{dis}$ defined above.




==> app_unification.tex <==
In Section \ref{sec:unification}, we briefly went through the
connections to our framework to several personalized FL methods. In
this appendix we provide a few more details related to these
connections.


\noindent\textbf{Regularization:} As noted earlier using
\eqref{eq:learning-log-generative-model} with the Gaussian population
prior connects to the use of $\ell_2$ regularizer in earlier
personalized learning works
\cite{dinh2020personalized,ozkara2021quped,hanzely2020federated,hanzely2020lower,li2021ditto},
which also iterates between local and global model estimates. This form can be explicitly seen in Appendix \ref{app:linear-regression}, where in Algorithm \ref{algo:personalized_regression}, we see that the Gaussian prior along with iterative optimization yields the regularized form seen in these methods. In these cases\footnote{One can generalize these by including $\sigmatheta^2$ in the unknown parameters.}, $\bbP(\Gamma)\equiv\calN(\vct{\mu},\sigmatheta^2\bbI_d)$ for unknown parameters $\Gamma=\{\vct{\mu}\}$. Note that since the parameters of the population distribution are unknown, these need to be estimated during the iterative learning process. In the algorithm, \ref{algo:personalized_regression} it is seen the $\vct{\mu}$ plays the role of the global model (and is truly so for the linear regression problem studied in  Appendix \ref{app:linear-regression}). 

\noindent\textbf{Clustered FL:} If one uses a \emph{discrete} mixture
model for the population distribution then the iterative algorithm
suggested by our framework connects to
\citep{zhang2021personalized,mansour2020approaches,ghosh2020efficient,smith2017federated,marfoq2021federated}. In
particular, consider a population model with parameters in the $m$-dimensional probability simplex
$\{\vct{\alpha}:\vct{\alpha}=[\alpha_1,\ldots,\alpha_k], \alpha_i\geq
0, \forall i, \sum_i\alpha_i=1\}$ which describing a distribution. If
there are $m$ (unknown) discrete distributions
$\{\mathcal{D}_1,\ldots,\mathcal{D}_m\}$, one can consider these as
the unknown description of the population model in addition to
$\vct{\alpha}$. Therefore, each local data are generated either as a
mixture as in \citep{marfoq2021federated} or by choosing one of the
unknown discrete distributions with probability $\vct{\alpha}$
dictating the probability of choosing $\mathcal{D}_i$, when hard
clustering is used (\emph{e.g.,} \citep{mansour2020approaches}). Each
node $j$ chooses a mixture probability $\vct{\alpha}^{(j)}$ uniformly
from the $m$-dimensional probability simplex. In the former case, it
uses this mixture probability to generate a local mixture
distribution. In the latter it chooses $\mathcal{D}_i$ with
probability $\vct{\alpha}^{(j)}_i$.

As mentioned earlier, not all parametrized distributions can be
written as a mixture of \emph{finite} number distributions, which is
the assumption for discrete mixtures. Consider a unimodal Gaussian
population distribution (as also studied in Appendix
\ref{app:linear-regression}). Since
$\bbP(\Gamma)\equiv\calN(\vct{\mu},\sigmatheta^2\bbI_d)$, for node
$i$, we sample $\vct{\theta}_i\sim \bbP(\Gamma)$. We see that the
actual data distribution for this node is
$p_{\vct{\theta}_i}(y|\vct{x})=\calN(\vct{\theta_i}^{\top}\vct{x},\sigma^2)$. Clearly
the set of such distributions $\{p_{\vct{\theta}_i}(y|\vct{x})\}$
\emph{cannot} be written as any finite mixture as
$\vct{\theta_i}\in\mathbb{R}^d$ and $p_{\vct{\theta}_i}(y|\vct{x})$ is
a unimodal Gaussian distribution, with same parameter $\vct{\theta_i}$
for all data generated in node $i$. Essentially the generative
framework of finite mixtures (as in \citep{marfoq2021federated}) could
be restrictive as it does not capture such parametric models.

\noindent\textbf{Knowledge distillation:} The population distribution
related to a regularizer based on Kullback-Leibler divergence
(knowledge distillation) has been shown in Appendix
\ref{app:adaped}. Therefore this can be cast in terms of information
geometry where the probability falls of exponentially with in this
geometry. Hence these connect to methods such as
\cite{lin2020ensemble,li2019fedmd,shen2020federated,ozkara2021quped},
but the exact regularizer used does not take into account the full
parametrization, and one can therefore improve upon these methods.

\noindent\textbf{FL with Multi-task Learning (MTL):} In this framework,
a \emph{fixed} relationship between tasks is usually assumed
\citep{smith2017federated}. Therefore one can model this as a Gaussian
model with \emph{known} parameters relating the individual models. The
individual models are chosen from a joint Gaussian with particular
(known) covariance dictating the different models, and therefore
giving the quadratic regularization used in FL-MTL
\citep{smith2017federated}. In this the parameters of the Gaussian
model are known and fixed.

\noindent\textbf{Common representations:} The works in
\cite{du2021fewshot,prateek2021differentially} use a linear model
where $y\sim\mathcal{N}(\vct{x}^{\top}\vct{\theta}_i,\sigma^2)$ can be
considered a local generative model for node $i$. The common
representation approach assumes that $\vct{\theta}_i=\sum_{j=1}^k
\mat{B}\vct{w}_j^{(i)}$, for some $k\ll d$, where
$\vct{\theta}_i\in\mathbb{R}^d$. Therefore, one can parametrize a
population by this (unknown) common basis %$\{\vct{b}_j\}$
$\mat{B}$, and under
a mild assumption that the weights are bounded, we can choose a
uniform measure in this bounded cube to choose $\vct{w}^{(i)}$ for
each node $i$. The alternating optimization iteratively discovers the
global common representation and the local weights as done in
\cite{du2021fewshot,prateek2021differentially} (and references
therein).

